TNO or Comet? The Search for Activity and Characterization of Distant Object 418993 (2009 MS9)

2009 MS9 is a trans-Neptunian object (TNO) whose perihelion brings it close to the distance where some long period comets are seen to become active. Knowing this, and the fact that this object appears to brighten in excess of it's predicted nucleus brightness suggests that 2009 MS9 has a delayed onset of activity brought on by the sublimation of a species more volatile than water. In this paper we characterize 2009 MS9's physical properties and investigate potential outgassing through composite images, sublimation models, and measurements of spectral reflectivity. We find that deep composite images of the object at various epochs along its orbit show no evidence of dust yet place sensitive limits to the dust production. We estimate the nucleus radius to be 11.5 km $\pm 3.5$ km using thermal IR modeling from NEOWISE data and use this and data pre-perihelion to estimate a geometric albedo of 0.25. We compare a CO-sublimation activity model to its post perihelion heliocentric light curve and find this data supports an active fractional area of $5 \times 10^{-6}$ assuming 2 $\mu$m sized grains and other typical comet parameters. The spectral reflectivity of the surface materials obtained with the Gemini Observatory and CFHT at different epochs shows a reddening spectral slope. We compare the physical properties of 2009 MS9 to both TNO and comet populations, and speculate that 2009 MS9's reddening may be due to the buildup of a dust mantle on the surface and could be an explanation of why TNOs exhibit a color bimodality.

==> Tab-Data.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccccl}
\tablecaption{Observing Geometry and Photometry \label{tab:data}}
\tablehead{
\colhead{UTDate                    } &
\colhead{JD\tablenotemark{a}       } &
\colhead{$r$\tablenotemark{b}      } &
\colhead{$\Delta$\tablenotemark{b} } &
\colhead{$\alpha$\tablenotemark{b} } &
\colhead{TA\tablenotemark{c}       } &
\colhead{Filt                      } &
\colhead{\# Images                 } &
\colhead{mag$\pm$$\sigma$          } &
\colhead{r$_{mag}$$\pm$$\sigma$\tablenotemark{d}} &
\colhead{Color/Comment}
}
\startdata
\multicolumn{11}{l}{\bf PanSTARRS1 data}\\
2010/06/04 & 5352.10123	& 28.665 & 28.754 & 2.017 & -151.16 & i$_{p1}$ &  2 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\
2012/08/07 & 6146.81325	& 25.061 & 25.146 & 2.306 & -149.01 & r$_{p1}$ &  2 & $<$21.8$\pm$0.3   & $<$21.8$\pm$0.3  & Limiting mag \\
2014/06/14 & 6821.46247 & 21.802 & 21.829 & 2.666 & -146.54 & i$_{p1}$ &  3 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\ 
2014/06/13 & 6822.51886 & 21.797 & 21.824 & 2.667 & -146.54 & i$_{p1}$ &  3 & $<$20.7$\pm$0.3   & $<$20.9$\pm$0.3  & Limiting mag \\
2014/07/05 & 6844.27742 & 21.688 & 21.729 & 2.681 & -146.45 & i$_{p1}$ &  2 & $<$20.8$\pm$0.3   & $<$21.0$\pm$0.3  & Limiting mag \\ 
2014/03/20 & 6737.07683 & 22.221 & 22.202 & 2.569 & -146.88 & r$_{p1}$ &  2 &    20.67$\pm$0.30 & 20.67$\pm$0.30 & \\
2014/09/08 & 6908.76850 & 21.364 & 21.430 & 2.692 & -146.17 & i$_{p1}$ &  4 &    20.60$\pm$0.05 & 20.77$\pm$0.05 & \\
2015/05/06 & 7149.01152 & 20.138 & 20.122 & 2.871 & -145.09 & i$_{p1}$ &  4 &    20.10$\pm$0.04 & 20.28$\pm$0.04 & \\
2015/05/07 & 7150.00904 & 20.133 & 20.117 & 2.872 & -145.08 & i$_{p1}$ &  4 &    20.27$\pm$0.05 & 20.45$\pm$0.05 & \\
2016/05/27 & 7536.02124 & 18.088 & 18.052 & 3.211 & -143.07 & r$_{p1}$ &  4 &    19.53$\pm$0.04 & 19.53$\pm$0.04 & \\
2016/06/19 & 7558.88673 & 17.963 & 17.938 & 3.242 & -142.94 & i$_{p1}$ &  3 &    19.37$\pm$0.08 & 19.54$\pm$0.08 & \\
2016/06/21 & 7560.93624 & 17.952 & 17.928 & 3.245 & -142.93 & i$_{p1}$ &  2 &    19.37$\pm$0.06 & 19.54$\pm$0.06 & \\
2016/07/18 & 7587.88946 & 17.805 & 17.803 & 3.270 & -142.77 & i$_{p1}$ &  4 &    19.53$\pm$0.05 & 19.71$\pm$0.05 & \\
2017/04/10 & 7854.05173 & 16.322 & 16.280 & 3.519 & -141.06 & i$_{p1}$ &  4 &    19.19$\pm$0.07 & 19.36$\pm$0.07 & \\
2017/05/21 & 7894.91140 & 16.089 & 16.019 & 3.604 & -140.77 & w$_{p1}$ &  4 &    19.45$\pm$0.03 & 19.39$\pm$0.03 & Discovery \\
2017/06/16 & 7920.97821 & 15.940 & 15.874 & 3.651 & -140.59 & i$_{p1}$ &  4 &    18.85$\pm$0.04 & 19.02$\pm$0.04 & \\
2017/06/25 & 7929.91675 & 15.888 & 15.828 & 3.666 & -140.52 & w$_{p1}$ &  4 &    19.19$\pm$0.03 & 19.13$\pm$0.03 & \\
2017/08/06 & 7971.88255 & 15.646 & 15.638 & 3.715 & -140.21 & i$_{p1}$ &  4 &    18.94$\pm$0.05 & 19.11$\pm$0.05 & \\
2017/08/17 & 7982.77565 & 15.583 & 15.594 & 3.721 & -140.13 & w$_{p1}$ &  4 &    19.02$\pm$0.01 & 18.97$\pm$0.02 & \\
2017/08/30 & 7995.76736 & 15.508 & 15.542 & 3.725 & -140.03 & i$_{p1}$ &  4 &    18.78$\pm$0.04 & 18.96$\pm$0.04 & \\
2017/09/07 & 8003.77876 & 15.461 & 15.511 & 3.724 & -139.96 & i$_{p1}$ &  4 &    18.72$\pm$0.04 & 18.90$\pm$0.04 & \\
2017/06/16 & 7920.95557 & 15.940 & 15.874 & 3.651 & -140.59 & r$_{p1}$ &  4 &    18.96$\pm$0.06 & 19.14$\pm$0.06 & \\
2017/07/05 & 7939.88379 & 15.831 & 15.779 & 3.681 & -140.45 & r$_{p1}$ &  2 &    18.94$\pm$0.14 & 19.11$\pm$0.14 & \\
2017/07/07 & 7941.90196 & 15.819 & 15.770 & 3.684 & -140.43 & r$_{p1}$ &  4 &    19.24$\pm$0.11 & 19.41$\pm$0.11 & \\
2017/07/15 & 7949.87944 & 15.773 & 15.733 & 3.694 & -140.37 & r$_{p1}$ &  4 &    18.82$\pm$0.06 & 19.00$\pm$0.06 & \\
2017/07/17 & 7951.90526 & 15.762 & 15.724 & 3.696 & -140.36 & r$_{p1}$ &  4 &    19.15$\pm$0.20 & 19.33$\pm$0.20 & \\
\hline
\multicolumn{11}{l}{\bf CFHT Archival data from CADC} \\
2013/05/12 & 6424.61132 & 23.744 & 23.767 & 2.436 & -148.07 & u        &  7 &    23.09$\pm$0.17 & 20.76$\pm$0.23 & \\
\hline
\multicolumn{10}{l}{\bf CFHT new data} \\
2017/05/24 & 7898.05595 & 16.071 & 16.000 & 3.610 & -140.75 & w        &  1 &    19.292$\pm$0.007 & 19.237$\pm$0.007 & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & g        &  1 &    19.673$\pm$0.015 & & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & r        &  1 &    19.155$\pm$0.015 & 19.155$\pm$0.015 & (g-r) = 0.52$\pm$0.02 \\
2017/06/24 & 7928.97060 & 15.894 & 15.833 & 3.665 & -140.53 & g        &  1 &    19.539$\pm$0.012 & & \\
2017/06/24 & 7928.97049 & 15.894 & 15.833 & 3.665 & -140.53 & r        &  1 &    19.067$\pm$0.013 & 19.067$\pm$0.013 & (g-r) = 0.47$\pm$0.02 \\
2017/07/16 & 7950.83854 & 15.768 & 15.729 & 3.695 & -140.37 & r        & 12 &    19.081$\pm$0.004 & 19.081$\pm$0.004 & \\
2017/07/25 & 7990.80063 & 15.768 & 15.729 & 3.695 & -140.37 & g        &  1 &    19.567$\pm$0.011 & & (g-r) = 0.56$\pm$0.02 \\
2017/07/25 & 7990.80285 & 15.768 & 15.729 & 3.695 & -140.37 & r        &  1 &    19.007$\pm$0.012 & 19.007$\pm$0.012 & \\
2017/07/26 & 7991.80022 & 15.537 & 15.562 & 3.724 & -140.06 & u        &  2 &    21.260$\pm$0.054 & & (u-r) = 2.33$\pm$0.06 \\
2017/07/26 & 7991.80602 & 15.531 & 15.558 & 3.724 & -140.06 & g        &  1 &    19.513$\pm$0.013 & & (g-r) = 0.59$\pm$0.02 \\
2017/07/26 & 7991.80407 & 15.537 & 15.562 & 3.724 & -140.06 & r        &  3 &    18.927$\pm$0.008 & 18.927$\pm$0.008 & \\
2017/07/26 & 7991.80889 & 15.531 & 15.558 & 3.724 & -140.06 & i        &  2 &    18.758$\pm$0.013 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.02 \\
2017/09/14 & 8010.74649	& 15.421 & 15.483 & 3.723 & -139.91 & g	       &  4 &    19.483$\pm$0.005 & & (g-r) = 0.55$\pm$0.01 \\
2017/09/14 & 8010.74282	& 15.421 & 15.483 & 3.723 & -139.91 & r	       &  2 &    18.932$\pm$0.009 & 18.932$\pm$0.009 & \\
2017/09/14 & 8010.74230	& 15.421 & 15.483 & 3.723 & -139.91 & i	       &  6 &    18.761$\pm$0.008 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.01 \\
2017/09/14 & 8010.75793	& 15.421 & 15.483 & 3.723 & -139.91 & z	       &  4 &    18.721$\pm$0.024 & & (r-z) = 0.21$\pm$0.03 \\
2017/09/15 & 8011.72479	& 15.415 & 15.479 & 3.723 & -139.90 & u	       &  3 &    20.995$\pm$0.039 & & (u-r) = 2.12$\pm$0.04 \\
2017/09/15 & 8011.74031	& 15.415 & 15.479 & 3.723 & -139.90 & g	       &  5 &    19.413$\pm$0.004 & & (g-r) = 0.54$\pm$0.01 \\
2017/09/15 & 8011.75514	& 15.415 & 15.479 & 3.723 & -139.90 & r	       &  2 &    18.873$\pm$0.007 & 18.873$\pm$0.007 & \\
\enddata
\tablenotetext{a}{Julian Date -2450000.0}
\tablenotetext{b}{Heliocentric, geocentric distance (au) and phase angle (deg).}
\tablenotetext{c}{True anomaly (deg), position along orbit, TA at perihelion=0$^{\circ}$}
\tablenotetext{d}{Magnitude and error through 5$''$ radius aperture.}
\tablenotetext{e}{Magnitude and error converted to SDSS $r$ as described in the text}
\end{deluxetable*}
\end{longrotatetable}


==> tab-geometry.tex <==
%\begin{longtable*}
\begin{deluxetable*}{cccccccl}
\tablecaption{\label{tab:geom}Observing Geometry}
\tablehead{
\colhead{UT Start$^{\dag}$}  &
\colhead{MJD$^{\dag}$}       &
\colhead{UT End  }           &
\colhead{MJD     }           &
\colhead{r$^{\ddag}$}        &
\colhead{$\Delta$$^{\ddag}$} &
\colhead{$\alpha$$^{\ddag}$} &
\colhead{Telescope}
}
\startdata
06/25/09 12:33 & 55007.52315 & --             & --          & 12.874 & 12.536 & 4.326  & CFHT        \\
07/19/09 08:32 & 55031.35569 & 07/19/09 08:35 & 55031.35787 & 12.814 & 12.456 & 4.316  & CFHT        \\
07/20/09 09:17 & 55032.38698 & 07/20/09 09:20 & 55032.38916 & 12.811 & 12.454 & 4.317  & CFHT        \\
08/19/09 08:10 & 55062.34091 & 08/19/09 09:10 & 55062.38256 & 12.736 & 12.435 & 4.398  & CFHT        \\
08/21/09 06:35 & 55064.27451 & 08/21/09 09:09 & 55064.38166 & 12.731 & 12.436 & 4.406  & CFHT        \\
09/13/09 05:40 & 55087.23661 & 09/13/09 05:50 & 55087.24317 & 12.675 & 12.475 & 4.493  & CFHT        \\
10/12/09 05:05 & 55116.21187 & 10/12/09 05:24 & 55116.22521 & 12.605 & 12.565 & 4.539  & CFHT        \\
10/17/09 05:13 & 55121.21783 & 10/17/09 05:22 & 55121.22374 & 12.593 & 12.582 & 4.536  & CFHT        \\
11/14/09 05:46 & 55149.24055 & 11/14/09 06:06 & 55149.25427 & 12.526 & 12.681 & 4.442  & CFHT        \\
11/16/09 05:48 & 55151.24175 & 11/16/09 05:59 & 55151.24956 & 12.521 & 12.688 & 4.431  & CFHT        \\
02/13/10 15:51 & 55240.66070 & 02/13/10 15:54 & 55240.66266 & 12.316 & 12.709 & 4.151  & CFHT        \\
03/17/10 15:26 & 55272.64333 & --             & --          & 12.246 & 12.554 & 4.375  & CFHT        \\
04/17/10 14:35 & 55303.60810 & --             & --          & 12.179 & 12.340 & 4.634  & CFHT        \\
06/12/10 09:18 & 55359.38817 & 06/12/10 12:25 & 55359.51794 & 12.063 & 11.908 & 4.801  & CFHT        \\
07/07/10 08:13 & 55384.34257 & 07/07/10 08:27 & 55384.35255 & 12.012 & 11.745 & 4.734  & CFHT        \\
07/15/10 10:00 & 55392.41723 & 07/15/10 14:57 & 55392.62323 & 11.996 & 11.701 & 4.705  & CFHT        \\
09/05/10 06:36 & 55444.27528 & 09/05/10 07:01 & 55444.29302 & 11.895 & 11.554 & 4.637  & CFHT        \\
09/11/10 07:12 & 55450.30016 & 09/11/10 09:12 & 55450.38359 & 11.884 & 11.554 & 4.650  & CFHT        \\
10/02/10 05:10 & 55471.21567 & 10/02/10 06:09 & 55471.25635 & 11.845 & 11.579 & 4.720  & CFHT        \\
10/03/10 05:23 & 55472.22454 & 10/03/10 06:24 & 55472.26733 & 11.843 & 11.581 & 4.724  & CFHT        \\
10/04/10 05:06 & 55473.21296 & 10/04/10 06:08 & 55473.25575 & 11.841 & 11.583 & 4.728  & CFHT        \\
10/05/10 05:17 & 55474.22055 & 10/05/10 06:35 & 55474.27496 & 11.839 & 11.585 & 4.732  & CFHT        \\
10/06/10 05:14 & 55475.21864 & 10/06/10 06:19 & 55475.26354 & 11.837 & 11.588 & 4.736  & CFHT        \\
12/03/10 04:33 & 55533.18989 & 12/03/10 04:35 & 55533.19155 & 11.733 & 11.818 & 4.778  & CFHT        \\
07/31/11 12:31 & 55773.52161 & 07/31/11 14:43 & 55773.61374 & 11.369 & 11.062 & 4.946  & CFHT        \\
08/01/11 08:51 & 55774.36906 & 08/01/11 09:37 & 55774.40070 & 11.368 & 11.056 & 4.939  & CFHT        \\
08/02/11 11:11 & 55775.46631 & 08/02/11 12:52 & 55775.53666 & 11.367 & 11.049 & 4.930  & CFHT        \\
07/04/13 14:04 & 56477.58615 & 07/04/13 14:49 & 56477.61803 & 11.027 & 11.159 & 5.210  & CFHT        \\
07/05/13 13:20 & 56478.55567 & --             & --          & 11.027 & 11.147 & 5.220  & CFHT        \\
07/06/13 13:32 & 56479.56404 & --             & --          & 11.027 & 11.136 & 5.230  & CFHT        \\
09/26/14 14:16 & 56926.59503 & 09/26/14 14:28 & 56926.60300 & 11.406 & 10.614 & 3.208  & CFHT        \\
02/06/16 05:08 & 57424.21413 & 02/06/16 05:10 & 57424.21587 & 12.300 & 12.527 & 4.431  & CFHT        \\
08/21/17 14:37 & 57987.10902 & 08/21/17 14:42 & 57987.11250 & 13.729 & 13.542 & 4.118  & CFHT        \\
09/13/17 14:51 & 58009.61895 & 02/06/16 14:53 & 58009.62082 & 13.815 & 13.199 & 3.378  & CFHT        \\
02/12/17 09:17 & 58099.38725 & 02/12/17 10:05 & 58099.42081 & 14.079 & 13.323 & 2.631  & CFHT        \\
02/13/18 05:50 & 58162.24318 & 02/13/18 05:52 & 58162.24505 & 14.268 & 14.499 & 3.826  & CFHT        \\
09/08/15 13:23 & 57273.55802 & 09/08/15 14:25 & 57273.60121 & 11.984 & 11.364 & 3.904  & Gemini      \\
11/08/16 11:46 & 57700.49097 & 11/08/16 11:56 & 57700.49734 & 12.965 & 11.988 & 0.757  & Gemini      \\
01/17/18 07:24 & 58135.30901 & --             & --          & 14.187 & 13.958 & 3.894  & Gemini      \\
11/10/18 12:07 & 58432.50503 & 11/10/16 14:01 & 58432.58434 & 15.113 & 14.144 & 0.806  & Gemini      \\
11/30/18 06:56 & 58452.28941 & 11/30/18 08:36 & 58452.35858 & 15.176 & 14.292 & 1.695  & Gemini      \\
08/14/11 21:45 & 55788.40650 & 08/14/11 22:03 & 55788.41880 & 11.351 & 10.974 & 4.828 & PS1          \\
08/19/11 20:03 & 55793.33550 & 08/19/11 20:51 & 55793.36890 & 11.345 & 10.949 & 4.789 & PS1          \\
08/22/11 19:05 & 55796.29550 & 08/22/11 19:55 & 55796.33050 & 11.341 & 10.935 & 4.766 & PS1          \\
09/26/11 18:19 & 55831.26320 & 09/26/11 18:38 & 55831.27670 & 11.300 & 10.851 & 4.638 & PS1          \\
08/15/12 23:09 & 56155.46510 & 08/15/12 23:56 & 56155.49790 & 11.042 & 10.646 & 4.929 & PS1          \\
10/16/13 19:34 & 56582.31560 & 10/16/13 19:50 & 56582.32680 & 11.074 & 10.312 & 3.442 & PS1          \\
09/20/13 21:42 & 56556.40430 & 09/20/13 22:00 & 56556.41710 & 11.060 & 10.369 & 3.897 & PS1          \\
10/04/13 06:46 & 56569.28194 & 10/04/13 09:25 & 56569.36528 & 11.067 & 10.320 & 3.566 & Lowell 1.8m  \\
10/05/13 09:03 & 56570.37708 & 10/05/13 09:32 & 56570.39722 & 11.068 & 10.318 & 3.547 & Lowell 1.8m  \\
\hline
\enddata
\begin{tablenotes}
\item[a] {\bf Notes:} $^{\dag}$Epoch of first and last exposures of each run, in UT and MJD = JD-2458000.5; $^{\ddag}$$r, \Delta$: helio- and geocentric distances, $\alpha$: solar phase angle (from Horizon ephemerides JPL\#10).
\end{tablenotes}
\end{deluxetable*}

